HumBugDB: A Large-scale Acoustic Mosquito Dataset

This paper presents the first large-scale multi-species dataset of acoustic recordings of mosquitoes tracked continuously in free flight. We present 20 hours of audio recordings that we have expertly labelled and tagged precisely in time. Significantly, 18 hours of recordings contain annotations from 36 different species. Mosquitoes are well-known carriers of diseases such as malaria, dengue and yellow fever. Collecting this dataset is motivated by the need to assist applications which utilise mosquito acoustics to conduct surveys to help predict outbreaks and inform intervention policy. The task of detecting mosquitoes from the sound of their wingbeats is challenging due to the difficulty in collecting recordings from realistic scenarios. To address this, as part of the HumBug project, we conducted global experiments to record mosquitoes ranging from those bred in culture cages to mosquitoes captured in the wild. Consequently, the audio recordings vary in signal-to-noise ratio and contain a broad range of indoor and outdoor background environments from Tanzania, Thailand, Kenya, the USA and the UK. In this paper we describe in detail how we collected, labelled and curated the data. The data is provided from a PostgreSQL database, which contains important metadata such as the capture method, age, feeding status and gender of the mosquitoes. Additionally, we provide code to extract features and train Bayesian convolutional neural networks for two key tasks: the identification of mosquitoes from their corresponding background environments, and the classification of detected mosquitoes into species. Our extensive dataset is both challenging to machine learning researchers focusing on acoustic identification, and critical to entomologists, geo-spatial modellers and other domain experts to understand mosquito behaviour, model their distribution, and manage the threat they pose to humans.

==> neurips_data_2021_resubmission.tex <==
\clearpage
\setcounter{section}{0}
\setcounter{page}{1}
\section{Resubmission document}
This paper is a resubmission from Round 1 at the NeurIPS 2021 Dataset and Benchmark Track. The previous submission, alongside reviews, author rebuttals, and meta-reviews are viewable on \url{https://openreview.net/forum?id=FNUijta5T-1}. 

We summarise the major revision which addresses the major criticism this paper received:
\paragraph{Key revision}
\begin{itemize}
\item[\xmark] The reviewers and meta-review collectively identified a lack of use cases, in particular data, features, and models for \textbf{mosquito species classification}.
\item[\cmark] To rectify this, we have added a \textbf{mosquito species classification task}, a \textbf{new baseline pre-trained on audio representations} (VGGish), and \textbf{an additional feature set}. As a result of the reviews, we have benchmarked 8 sets of model-feature combinations for a mosquito event detection task and 40 for mosquito species classification (5 sets of random seeds for all 8 combinations).
\end{itemize}



In this supplement, we will explain in more depth the key criticism responsible for the decision, along with the major change made to address this point in Section \ref{sec:Resubmission_key_revision}. Section \ref{sec:resubmissionChangelog} then provides a changelog with contributions sorted in order of importance. Section \ref{sec:resubmissionRebuttal} shows the specific changes made in response to every individual point raised by the reviewers.

\textcolor{red}{For ease of readability, every comment made by either reviewer or area chair is marked in red}.

\textcolor{ForestGreen}{Every comment made in response by the authors is marked in green. \textbf{Actions taken are further given in bold.}}


\subsection{Key revision}
\label{sec:Resubmission_key_revision}




The overall decision was justified with the following meta-review: 
\begin{pquotation}{Meta-review, Area chair}
\textcolor{red}{
`Although the paper proposed a dataset for an extremely important and relevant issue, reviewers felt that the final task the authors wanted to solve was not evaluated. There is a gap between the motivation (insect surveillance) and the task that is evaluated using the dataset (background removal).'}
\end{pquotation}

We are pleased that the area chair deems our dataset as a contribution to an extremely important and relevant issue, and we have carefully crafted a \textbf{new task for this re-submission} to ensure no gap between motivation and evaluation is left.

In more detail, we believe this remark stems from the compilation of the following reviewer comments, which all identified a lack of additional use cases and further baselines as a key area for improvement:

\begin{pquotation}{Mh2C review, Weakness 1}
\textcolor{red}{`There is a tremendous mismatch between the paper motivation and the technical part. The motivation is about mosquito surveillance, including automatic recognition of species. The benchmark is about differentiating mosquito signals from background noise, a much less interesting task.'}
\end{pquotation}

\begin{pquotation}{UKo3 review, Weaknesses summary}\textcolor{red}{`Overall this dataset suffers from baseline evaluations which are necessary to understand the usability of the dataset. I would ideally like to see more rigorous evaluations and more experiments to focus on how the dataset can be used.'}
\end{pquotation}

\begin{pquotation}{mM4X review, Weaknesses summary}\textcolor{red}{`Are there other/more applications that your data allows? It would be good to discuss more applications and do more benchmarking on them if possible.'}
\end{pquotation}


We have updated our work significantly to include models which are benchmarked for mosquito species classification. This new task is denoted Mosquito Species Classification (MSC) throughout the text. We have already rebutted the quote which unfairly categorises our initial work as simple background removal (see specific comments in {\ref{sec:reviewerMh2C}), whereas our work involved the careful creation of a mosquito event \textit{detection} task (MED), in which mosquito acoustic events are identified within the negative control class which includes other insects, animals, domestic, urban and rural scenes, speech, and many more acoustic events. With the inclusion of this new MSC task in addition to MED, we have covered the primary use cases which this dataset motivates comprehensively. Moreover, we have added an additional model (VGGish pre-trained on audio representations from AudioSet), and features (the input pipeline of VGGish log-mel features), to produce 8 sets of model-feature combinations for MED and 40 for MSC (5 sets of random seeds for all 8 combinations).




Additionally, we have expanded on potential use cases in Appendix \ref{sec:appendix_datasheet_uses} as:
\begin{enumerate}
    \item \textbf{Validating species classification models from the literature.}
\item \textbf{Frequency analysis.} Identifying the fundamental and harmonic frequencies of flight tone for a particular species, to improve upon the understanding of bioacoustics literature, and entomological research.
\item \textbf{Examining inter-species (or similar) variability.} For example, the effect on the sound of flight as a result of age, gender, or any field supported in the database.
\end{enumerate}

In the next section we will provide a full changelog from the past submission in order of significance. Section \ref{sec:resubmissionRebuttal} then gives  the full details of specific changes made in response to every point made by the reviewers.

\subsection{Changelog}
\label{sec:resubmissionChangelog}
\begin{enumerate}
    \item Added a species classification task, updated every section of the text accordingly (including new schematic diagram), and re-structured the paper to include baseline feature-model combinations for:
    \begin{enumerate}
        \item Mosquito Event Detection (MED)
        \item Mosquito Species Classification (MSC)
    \end{enumerate}
    \item Added VGGish \textit{model} baseline to both tasks
    \item Added VGGish \textit{features} as a baseline for both tasks
    \item Benchmarked the additional models and features to produce 8 sets of model-feature combinations for MED and 40 for MSC (5 sets of random seeds for all 8 combinations)
    \item Explained the motivation behind the two feature sets supplied in this paper as features which have been successfully used in the past for similar tasks (Feat. B), alongside VGGish features which act as a baseline (Feat. A).
    \item Re-worked literature review:
    \begin{enumerate}
        \item Table to compare notable datasets in the literature, more clearly illustrating the unique value of our data
        \item Split discussion into opto-acoustic and acoustic approaches to more clearly explain the context of our contribution and avoid any potential unfair treatment of relevant prior work.
        \item Amended and moved “state-of-art” comment to acoustic approaches comparison to not discredit any of the approaches utilising opto-acoustic sensors.
        \item Made clearer the need for longer recording samples for acoustic detection of mosquitoes in free flight with acoustic sensors.
        \item Added passage on mosquito biodiversity
    \end{enumerate}
    \item More clearly motivated the need for this data for insect monitoring with acoustic devices in Introduction
    \item Added Table \ref{tab:appendix_species} with species distribution per recording location to improve clarity of Figure \ref{fig:species_dist}.
    \item (Further) additional use cases:
    \begin{enumerate}
        \item Past use cases of this dataset added (Appendix \ref{sec:appendix_datasheet_uses}) and now referenced in text. Also made clear the Thailand (2018) data has been used in published work before in Section \ref{sec:wild}, and that MSC with Tanzania (2020) is an extension of that work.
        \item Visibility of related work improved with better hyperlinks to data and code repositories (Appendix \ref{sec:appendix_datasheet_uses})
        \item Greatly expanded on potential use cases (Appendix \ref{sec:appendix_datasheet_uses})
        \item Referenced use cases in the paper structure overview (Introduction), and in the introductory paragraph of Section \ref{sec:benchmark}.
    \end{enumerate}
    \item Added section on data bias \ref{sec:appendix_datasheet_databias}:
    \begin{enumerate}
        \item When discussing statistics of the datasets for training benchmark models (Section \ref{sec:benchmark}), we direct the reader to the new data bias section (\ref{sec:appendix_datasheet_databias}).
        \item Nature of mosquitoes: wild and lab grown
        \item Recording device
        \item Data imbalance
    \end{enumerate}
    \item Re-worded section on intended use cases of data in Section \ref{sec:humbug} to better link with Section \ref{sec:benchmark} and \ref{sec:appendix_datasheet_uses} to bulletproof the contributions and scope of our paper.
    \item Improved reference to \citet[Sec.\,2.1.2]{2021MEE} explaining bednets and mosquito behaviour
    \item Added detail on recording devices in Appendix \ref{sec:appendix_datasheet_collection} and linked in text
    \item Corrected reference to Appendix \ref{sec:appendix_testPerformance} which discusses Test Set B further
    \item Added motivation for BNN model classes in benchmark Section \ref{sec:benchmark}.
    \item Added further detail in Section \ref{sec:Task1_MED} to explain the difficulty of Test B in terms of SNR and recording environment.
    \item Expanded on database maintenance policies in Appendix \ref{sec:appendix_database_maintenance}.
    \item Improved baseline performance of MED models with Test B Feat. B.
\end{enumerate}

% \clearpage
\subsection{Full rebuttal and list of changes}
\label{sec:resubmissionRebuttal}

\subsubsection{Review scores}

\begin{table}[h]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Reviewer             & UKo3   & Mh2C & XGcR   & mM4X \\ \midrule
Score                & 4   & 6 & 5   & 9 \\
Response to Rebuttal(s) & \xmark   & \cmark (\xmark) & \xmark   & \cmark \\ \bottomrule
\end{tabular}
\end{table}



\subsubsection{Reviewer UKo3}
Access on: \url{https://openreview.net/forum?id=FNUijta5T-1&noteId=_gpXP9bnrE}.
\begin{pquotation}{UKo3, Weaknesses}
\textcolor{red}{`The authors should describe the modifications they made to a bed net that attracted mosquitos to fly close to the smartphone. The authors should also describe mosquito behavior that they exploited instead of just citing previous research work. I did not find the previous work online and was not able to verify this step.'}
\end{pquotation}
\begin{pquotation}{Authors, Weaknesses rebuttal}
\textcolor{ForestGreen}{In lines 127 and 179 of the original submission we have cited Sinka et al., 2021 which answers this question and offers citations for mosquito behaviour. \textbf{To make this information more easily accessible we added “Section 2.1.2” ([Sinka et al. 2021, Sec. 2.1.2]) to any citation made with reference to the adapted bednet.}}
\end{pquotation}

\begin{pquotation}{UKo3, Weaknesses}
\textcolor{red}{
Multiple parts of the data are actually recorded using a Telinga. Some description about this device and its usage for this project will be necessary for Section 3.}
\end{pquotation}

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{
`Section 3 describes the deployment pipeline, in which smartphones are the target. The Telinga device, however, was used to collect previous data (described in Section 4). \textbf{We added more detail on recording devices for the Datasheet for Datasets Appendix D.3 and cite this section in the paper upon first mention of the Telinga device.}'}
\end{pquotation}

\begin{pquotation}{UKo3, Weaknesses}
\textcolor{red}{
`The baseline models should be renamed appropriately. More baselines like VGG16 and Inception Net should probably be tried. I also believe, finetuning (transfer learning) on VGG16 trained on other audio-related tasks will be interesting and can improve performance.'}
\end{pquotation}

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{`The ResNet50 application is already a transfer learning paradigm (described in Appendix B.4. PyTorch ResNet-X), and is commonly encountered in literature. \textbf{Furthermore, we have added VGG16 pre-trained on audio specifically to the list of models that we trial.} Overall, the feature pipeline used as input to VGG16 has helped ResNet learn better representations for the MED task, and the model itself also performed well, but has not come out on top for either task (see Table 3 and Table 4). Nevertheless, we find it makes a useful addition to our codebase and we appreciate that users may be more familiar with this architecture over others. We would like to re-emphasise that this is a \textbf{dataset paper primarily and not a benchmark paper}: there is no requirement to evaluate so many features and models in the first place.}
\end{pquotation}


\begin{pquotation}{UKo3, Weaknesses}
\textcolor{red}{The performance of the models also varies widely in the two test sets. Detailed experiments should be done to analyze this. Furthermore, ResNet-18 and ResNet-50 are essentially similar architectures, with ResNet-50 being deeper. However, the trend of both of these models reverses in Set B when compared to Set A for ROC-AOC. Why is this happening?}
\end{pquotation}

This criticism is no longer relevant as experiments were re-done with many additional models and features. However, ROC scores are still significantly lower on Test B than Test A, which we explain in the main text. Our original rebuttal is still relevant, and hence we include this below:

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{`The TPR of all three models is <30\% on Test B, indicating the failure mode for all the models is consistent. The behaviour of all the models is also consistent across Test A. We have conducted further experiments with Test B to ensure data integrity and included these in Appendix B.5, which we explain in Section 5.3. \textbf{We note that our reference originally pointed to Appendix B.4, which was a typo we corrected to B.5.} The purpose of the inclusion of Test B as a true out of sample test, is that it represents an unpredictably difficult scenario that the models are likely to encounter in deployment.}
\end{pquotation}

\begin{pquotation}{UKo3, Weaknesses}\textcolor{red}{
`In line 324, the authors mention prior works which were not mentioned in the table. In my view, even they should be mentioned in the table, and their performance should be reported on this dataset.'}
\end{pquotation}

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{
`We cannot include that model in the same table as it has been designed and trained on one part of Test B and evaluated on another part. In this paper, however, Test B is held out completely from training (as you identify as Strength 4). The accuracy figures of the cited prior work are only a like-for-like comparison with Appendix B.5, where similar performance was observed, even though the prior model was tuned to that dataset.'}
\end{pquotation}

\begin{pquotation}{UKo3, Weaknesses}\textcolor{red}{`The species distribution is not clear in the graphs given in Figure 6 (supplementary material). Also, it will be really beneficial to have some information about the disease caused by each of these species. By reading the paper, I felt that only malaria-causing species were considered while opportunities existed to focus on other diseases like Dengue.'}
\end{pquotation}

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{
`\textbf{On the clarity of Figure 6, we added Table 6 showing the exact figures of species distribution per recording location and modality.} In line 188 of the original submission (Section 4.2.1) we specifically list the vectors of each disease: “These include primary malaria vectors (e.g. Anopheles gambiae, An. arabiensis), arbovirus vectors including primary vectors of dengue virus (Aedes albopictus), yellow fever virus (Aedes aegypti) and west nile virus (Culex quinquefasciatus).”'}
\end{pquotation}

\begin{pquotation}{UKo3, Weaknesses}\textcolor{red}{`No clear policies and strategies for dataset maintenance and update are mentioned in the paper. The dataset can and should be improved over time with more species, more data per species, etc.'}
\end{pquotation}

\begin{pquotation}{Authors, Weaknesses rebuttal}\textcolor{ForestGreen}{`Database maintenance in accordance with NeurIPS guidance on Datasheets for Datasets is described in Appendix D.6. We used a repository which resolves to the latest version with one DOI, and GitHub commits will be made for updated metadata and code. New data with species information is expected soon (recorded in the DRC), though due to COVID-19 no exact timelines can be supplied.'}
\end{pquotation}

\begin{pquotation}{UKo3, Additional feedback}\textcolor{red}{
\begin{enumerate}
    \item `Please put a small table in the related works comparing each dataset in terms of hours, expertize in labelling, background noise present or not, etc. It is very helpful for the reader to get the summary along with the long text in the related works section.'
\item `I did not understand the usage of Keras BNN and PyTorch ResNet BNN. Both the libraries support similar applications and could have been implemented using a common library.'
\end{enumerate}}
\end{pquotation}

\begin{pquotation}{Authors, Additional feedback rebuttal}\textcolor{ForestGreen}{
\begin{enumerate}
    \item `This is an excellent suggestion. \textbf{To clarify our contribution relative to related works, we re-wrote Related Work and added Table 1 which lists the data source, the number of samples, the sample duration, the sensor, the number of species, and the type of mosquito surveyed.}'
\item `The strong point of the code framework is that both libraries are natively supported with a common interface. This leaves practitioners free to choose whichever framework they are most comfortable with. We would be happy to port the keras model to PyTorch if it improves uptake in future.'
\end{enumerate}}
\end{pquotation}

\begin{pquotation}{UKo3, Clarity}
\textcolor{red}{`Overall the writing quality should be improved to make the contributions clearer.'}
\end{pquotation}

\begin{pquotation}{Authors, Clarity rebuttal}\textcolor{ForestGreen}{`\textbf{We have reiterated our contributions in the Contributions section, and added our motivation for using acoustic devices in the Introduction.}'}
\end{pquotation}

\subsubsection{Reviewer Mh2C}
\label{sec:reviewerMh2C}
\paragraph{Initial review and rebuttals:} \url{https://openreview.net/forum?id=FNUijta5T-1&noteId=MJ1SgNBBT_2}.
\begin{pquotation}{Mh2C, Weaknesses}\textcolor{red}{`There is a tremendous mismatch between the paper motivation and the technical part. The motivation is about mosquito surveillance, including automatic recognition of species. The benchmark is about differentiating mosquito signals from background noise, a much less interesting task.'}
\end{pquotation}


\begin{pquotation}{Mh2C, Weaknesses}\textcolor{red}{`The paper lacks a clear explanation of why Test B is so challenging that makes the tested models fail. How is this data partition relevant?'}
\end{pquotation}

\begin{pquotation}{Author response}\textcolor{ForestGreen}{`We state reasons for the challenge Test B poses in the first paragraph of Section 5. Furthermore, as the set of data is a test set, it acts as an independent verification to build robust models. We ensured the data is correct, for which we discuss in Section 5.3. The data partition is relevant directly, and critically, as our experiments we supply in Appendix B.5 show that when training on a held-out part of Test B, model performance is more than adequate. However, when the set is disparate to the remaining training data, all of the baselines are unable to achieve good classification performance. Data partitioning is crucial to understanding model performance, which is why we emphasise it so strongly throughout the text. As real-life recordings are often unpredictable, this makes Test B a good candidate as a test-bed for further research.}
\end{pquotation}

\textbf{Since the rebuttal we have added further detail in Section \ref{sec:Task1_MED} to explain the difficulty of Test B in terms of SNR and recording environment.}}



\begin{pquotation}{Mh2C, Weaknesses and Clarity}\textcolor{red}{
`The main article flaw is a tremendous mismatch between motivation and reality. The motivation regarding mosquito recognition is highly engaging, but the dataset is about background noise identification. There is nothing in the text discussing data, features or models for species identification.'
`The main article flaw is a tremendous mismatch between motivation and reality. The motivation regarding mosquito recognition is highly engaging, but the dataset is about background noise identification. There is nothing in the text discussing data, features or models for species identification.'}
\end{pquotation}
\begin{pquotation}{Author rebuttal to Mh2C}
\textcolor{ForestGreen}{`Species recognition is important, but can only be performed if a suitable mosquito detector is part of the pipeline. Therefore, our paper motivation is not at all a "tremendous mismatch", but instead a vital component of a real-world predictive pipeline. The database is focused on identifying mosquitoes within the background and on real-world applications of low-cost acoustic sensing in communities in which the disease is prevalent. It is the difficulty of detecting the mosquitoes within noisy backgrounds that motivates us to provide benchmarks for this task.'}
\end{pquotation}

\textbf{Since the rebuttal, we have further added points 1 to 5 of the Changelog (\ref{sec:resubmissionChangelog}) to address the lack of discussion about features and models for species identification.}


\begin{pquotation}{Mh2C Relation to Prior Work}{\color{red}
The article covers a relevant part of the literature, but it misses a few spots. One example is that the first set of pseudo-acoustic data was released as part of a machine learning competition and is available at the UCR Flying Insect Classification Using Inexpensive Sensors website.

 I disagree with the paragraph (85-92) about the work of Fanioudakis et al. Could you explain what "lack of typical background acoustic properties" means? Their work sounds like a better approach for collecting this data since those sensors are insensitive to external factors that generate background noise. Therefore, the problem this paper/benchmark/dataset proposes to solve inexists with data collected with those sensors. Also, the statement about "state-of-the-art" models is very misleading, given the references are for music recognition models, which are naturally designed to work with long samples. However, there are plenty of models that can work with shorter signals.}
 \end{pquotation}
 
 
 \begin{pquotation}{Author rebuttal for Relation to Prior Work}{\color{ForestGreen} `As to a “lack of typical background properties”, the inclusion of background noise addresses the sentiments of Vasconcelos et al., who published their view:'

``Finally, none of the published datasets includes environmental noise ..., which is essential to fully characterize mosquitoes in real world scenarios.''

`For training methods using purely acoustic approaches, a control group of background environmental recording is required to test whether the models are learning the mosquito acoustics or the background conditions.

We can see how the “state-of-art models” comment may come across as misleading. \textbf{We have amended and moved this statement to the acoustic approaches comparison to not discredit any of the approaches utilising opto-acoustic sensors, where those “state-of-art” models would not be useful}.

Furthermore, the opto-acoustic datasets of Chen et al., Fanioudakis et al. use cages of lab raised mosquitoes - these will lack the natural variation found in wild captured specimens [Huho et al., 2007, Hoffmann and Ross, 2018]. This limits the use of their data for the identification of wild populations. \textbf{We have included this in the Related Work section}.'}
 \end{pquotation}
 
 
 \begin{pquotation}{Mh2C, Ethics}\textcolor{red}{
 I do not foresee any ethics issues. Most countries do not require ethical approval for experimental work with live insects.} \end{pquotation}

We did not respond to this comment originally, but note that it is dismissive of \textbf{essential} proper ethical protocol, which we followed and documented in Section \ref{sec:appendix_datasheet_collection}. 

\paragraph{Reviewer response and further rebuttal:} \url{https://openreview.net/forum?id=FNUijta5T-1&noteId=5VKg_68FzIK}

 \begin{pquotation}{Mh2C response}\textcolor{red}{`It is clear from the text that segmentation is a previous necessary step for species recognition. My complaint is not that the segmentation is irrelevant in the pipeline, but the text virtually ignores the segmentation problem. It comes as a "surprise" in section 4 when it becomes clear that the task addressed in the paper is not species recognition but the separation of signal and background noise... I am assessing this particular paper with its claims and contributions. If the paper "sells" the idea of species recognition, I expect this paper to shows a dataset and models for this end.'}
\end{pquotation}

\textbf{We have addressed this in our key revision as discussed previously (see Changelog \ref{sec:resubmissionChangelog} points 1 to 5).}


 \begin{pquotation}{Mh2C response}\textcolor{red}{`Thanks for this quote. I took a bit of time to check the mentioned paper, and this passage comes with no citation of any source and no supporting experimental evidence. The passage mentions that including wind noise would help to recognise different species. Could you explain how ambient noise such as wind is relevant to species recognition and what evidence you have to support the original claim in your paper? Otherwise, it seems you are reverberating unsupported claims from other papers.'}
 \end{pquotation}
 
  \begin{pquotation}{Author response}{\color{ForestGreen}
 `Your statement of:

\textcolor{red}{``The passage mentions that including wind noise would help to recognise different species.''}

is misrepresenting the statement made by the original authors (whose work has been peer reviewed and published). To provide better context for their statement, we quote:

``One crucial research question ... is to what extent the changes induced by environmental conditions (location, temperature, time of day, humidity, air density, etc.) impact the pattern recognition algorithms. The availability of public datasets collected in different geographic and environmental conditions is critical to understanding how these issues affect recognition algorithms. Finally, none of the published datasets includes environmental noise (e.g. wind or ambient noise), which is essential to fully characterize mosquitoes in real world scenarios.''

We believe the authors are emphasising the need for noisy, real-world data for the purpose of training, evaluating and deploying robust models. This is exactly what we provide in this dataset.

By supplying background from the same source, we help build balanced classes for the models, and further provide a control group for scientific investigation. If we use different data sources for background, we introduce additional variables which will lead to confounding when assessing the model's ability to identify mosquito events. An extra utility of this background is that it is sourced from real-world field studies, which is typical of the locations of deployment for this device class. This data is essential for building more robust models for ongoing and future trials.'}
\end{pquotation}

 \begin{pquotation}{Mh2C response}\textcolor{red}{`The explanation in Section 5 is ``very difficult low-SNR'' and ``prominent species not as well represented''. Apart from being an imprecise explanation, my question was why it is the case. What makes this data partition particularly interesting for assessment, and why one should invest their time improving performance in this set?}
 \end{pquotation}
 
   \begin{pquotation}{Author response}{\color{ForestGreen}
   `The dataset shows a failure mode of common models trained on a large quantity of data. It is precisely this negative result that makes this dataset interesting: if we were able to build models in the past that were trained on parts of this data, that perform excellently on the remaining parts, why do models struggle to generalise to this dataset when it is completely withheld? This is an excellent test for robustness: the varying nature of the background and signal, though to our ears as humans does not pose a challenge to labelling, is proving very difficult for the models. This is a research question we motivate with this test set. We hoped to present this as a case example of difficult subsets of test data to inspire improved methods.'}
   \end{pquotation}
   
 
 \subsubsection{Reviewer XGcR}
 Access on: \url{https://openreview.net/forum?id=FNUijta5T-1&noteId=vk9cFFUOarR}.
 We would like to preface by mentioning this review was unconstructive, and of severely sub-standard quality. It was thus reported to the event organisers and area chairs. Nevertheless, we will include their original feedback and our response for completeness.
 \begin{pquotation}{XGcR Weaknesses}\textcolor{red}{`The quantification and visualization of statistics and comparisons of datasets are relatively limited.'}
 \end{pquotation}
 
 \begin{pquotation}{Author response, Weaknesses}{\color{ForestGreen}
 `This is a unique dataset, in terms of its size, extent and laborious real-world collection. Comparison with like-for-like data is therefore not easy. What visualization and statistics are you looking for? Please detail your request. We are in the process of adding a table with related datasets (as per Reviewer 1 and 2's request) and will respond once the changes have been made.'}
 \end{pquotation}
 
  \begin{pquotation}{XGcR Weaknesses}\textcolor{red}{`I believe such a paper can be well published in a mid-ranked conference but I do not see a sufficient novel contribution to NeurIPS. It is one more vanilla dataset.'}
  \end{pquotation}
  
   \begin{pquotation}{Author response, Weaknesses}{\color{ForestGreen}
 `Your comment is conjecture, dismissive and at odds with the other reviewers (even those who are constructively critical of the submission). We are aghast with your comment about vanilla datasets. This seems highly dismissive of the years of careful work that has gone into mosquito research and data collection, not just by us, but by many others as well. As to the relevance of the research, we suggest you consider how little data is available to disease (malaria) specialists about the range and activity of mosquitos. Indeed, for some parts of the world, entire policies are based on very small amounts of data. Please also consider that malaria alone is responsible for >400,000 deaths every year in Africa (COVID deaths in Africa are currently [July 2021] around approx 150,000 and no one would call that irrelevant or ‘vanilla’). This dataset is of remarkable size and variation and nothing like it exists. We will certainly make this clearer by including a table of related datasets with useful statistics in the Related Work section (in response to comments made by all reviewers). No prior research has engaged so extensively with field trials in global rural communities to collect data “in the wild” -- previous reliance on lab-cultured mosquitoes does not provide real-world data. The data we and colleagues have collated has the potential to make a difference -- in the way mosquitoes are monitored, and intervention policies are created and assessed.'}
 \end{pquotation}

  \begin{pquotation}{XGcR, Relation to Prior Work}\textcolor{red}{`There should be more clear quantification and visualization about the difference from prior work.'}
  \end{pquotation}
  \textbf{These have been addressed in point 6 of the changelog \ref{sec:resubmissionChangelog}}.

\begin{pquotation}{XGcR, Documentation}\textcolor{red}{`There are some limitations regarding the application of the proposed dataset.'}
\end{pquotation}

\begin{pquotation}{Author response}\textcolor{ForestGreen}{
What are the limitations you state and how are they relevant to documentation? We provided a very extensive Datasheet for Datasets and have documented all of our code and data to the best of our knowledge and ability.}
\end{pquotation}

 \subsubsection{Reviewer mM4X}
Access on: \url{https://openreview.net/forum?id=FNUijta5T-1&noteId=sdAyQWi0nw}

\begin{pquotation}{mM4X, Weaknesses}{\color{red}
`I don't have any big concern preventing me from accepting this paper, but below are some minor points if authors want to further improve the work:

\begin{enumerate}
    \item Can you discuss the data bias? I understand that it's not possible to collect such natural data without any bias. But some discussion about the data bias (e.g. different countries, data imbalance on species), and how would it affect the network training for applications, and how do you practically address these data bias issues, will be very interesting to the readers.
\item Are there other/more applications that your data allows? It would be good to discuss more applications and do more benchmarking on them if possible.'
\end{enumerate}}
\end{pquotation}

\begin{pquotation}{Author response, Weaknesses}{\color{ForestGreen} 

\begin{enumerate}
    \item `\textbf{Data bias}:
we have added an extensive section (D.6) to describe sources of data bias and mitigation strategies for a range of use cases:
\begin{itemize}
\item Nature of mosquitoes: wild and lab grown
\item Recording device
\item Data imbalance
\end{itemize}
\item \textbf{Additional applications}: Appendix D.5 has now been re-worked as follows:

\begin{itemize}
\item \textbf{Past use cases of this dataset added and now referenced in text. }
\item Visibility of related work improved with better hyperlinks to data and code repositories.
\item Greatly expanded on the following potential use cases:
\begin{itemize}
\item \textbf{Species classification with HumBugDB}. Training a machine learning model to distinguish between various species. \textcolor{black}{\normalfont{\textbf{Post-rebuttal moved to main text for Revision 2, see Changelog \ref{sec:resubmissionChangelog} points 1 to 5.}}}
\item \textbf{Validating species classification models from the literature}.
Frequency analysis. Identifying the fundamental and harmonic frequencies of flight tone for a particular species, to improve upon the understanding of bioacoustics literature, and entomological research.
\item \textbf{Examining inter-species (or similar) variability}. For example, the effect on the sound of flight as a result of age, gender, or any field supported in the database.
\end{itemize}
\end{itemize}
\end{enumerate}
To ensure these useful resources do not go unnoticed in the main text, we linked these new sections as follows:

\textbf{Referenced additional use cases (D.5) in the paper structure overview (Introduction), and in the introductory paragraph of Section 5.
When discussing statistics of the datasets for training benchmark models (Section 5, paragraph 1), we direct the reader to the new data bias section (D.6).'}}
\end{pquotation}
